SHIRO: Near-Optimal Communication Strategies for Distributed Sparse Matrix Multiplication

Distributed Sparse Matrix-Matrix Multiplication (SpMM) is a fundamental operation in high-performance computing and deep learning applications. The major performance bottleneck in distributed SpMM lies in substantial communication overhead, which limits both performance and scalability. In this paper, we identify two key sources of communication inefficiency in distributed SpMM: redundant data transfer due to sparsity unawareness, and suboptimal utilization of hierarchical network topology. To address these, we propose (1) a fine-grained, sparsity-aware communication strategy that reduces communication overhead by exploiting the sparsity pattern of the sparse matrix, and (2) a hierarchical communication strategy that maps the sparsity-aware strategy onto two-tier GPU network architectures, minimizing redundant data movement across slower inter-node links. We implement these optimizations in a comprehensive distributed SpMM framework, \method{}. Extensive evaluations on real-world datasets show that \method{} demonstrates strong scalability up to 128 GPUs, achieving geometric mean speedups of 221.5$\times$, 56.0$\times$, 23.4$\times$, and 8.8$\times$ in SpMM over four state-of-the-art baselines (CAGNET, SPA, BCL, and CoLa, respectively) at this scale.

==> figures/algorithm1.tex <==
{
% \captionsetup[algorithm]{skip=300pt, font=small}
% \setlength{\intextsep}{0pt}

\makeatletter
% \renewcommand{\@algocf@pre@ruled}{}
\renewcommand{\@algocf@post@ruled}{}
% \renewcommand{\@algocf@capt@ruled}{}
\renewcommand{\@algocf@pre@plain}{}
\renewcommand{\@algocf@post@plain}{}
\makeatother
\makeatletter
\setlength{\algomargin}{0pt} % remove algorithm2e’s side indent
\makeatother

\begin{algorithm}[t!]
\caption{Hierarchical Group Communication for Distributed SpMM (per-process view)}

\label{alg:hierarchical}
\footnotesize
% \begin{algorithmic}
\KwIn{Local sparse matrix blocks $\mathbf{A}_{row}$, $\mathbf{A}_{col}$; Dense matrix $\mathbf{B}$; Group ID $g_{id}$}
\KwOut{$B_{dist}$ (column-based communication result), $C_{recv}$ (row-based communication result)}

\textcolor{blue}{\textit{I.\circled{1}: Inter-group B fetch (Column-based)}}\\
\For{each group $g \neq g_{id}$}{
    $B_{send}^g \leftarrow$ CollectRequiredRows($g$, $\mathbf{A}_{col}$, $\mathbf{B}$)\\
    InterGroupSendRecv($B_{send}^g$, $B_{recv}^g$, $g$) \hfill $\triangleright$ Non-blocking
}

\textcolor{blue}{\textit{I.\circledwhite{1}: Intra-group C aggregation (Row-based)}}\\
$C_{row} \leftarrow$ SpMM($\mathbf{A}_{row}$, $\mathbf{B}$)\\
IntraGroupAlltoall($C_{row}$, $C_{partial}$)

\textcolor{blue}{\textit{II.\circledwhite{2}: Inter-group C transmission (Row-based)}}\\
\For{each group $g \neq g_{id}$}{
    $C_{agg}^g \leftarrow$ Aggregate($C_{partial}$, $g$)\\
    InterGroupSendRecv($C_{agg}^g$, $C_{recv}^g$, $g$) \hfill $\triangleright$ Non-blocking
}

\textcolor{blue}{\textit{II.\circled{2}: Intra-group B distribution (Column-based)}}\\
WaitRecv($B_{recv}$) \hfill $\triangleright$ Wait for Stage I.\circled{1}\\
IntraGroupAlltoall($B_{recv}$, $B_{dist}$)\\
WaitRecv($C_{recv}$) \hfill $\triangleright$ Wait for Stage II.\circledwhite{2}\\

\Return{$B_{dist}$, $C_{recv}$}
% \end{algorithmic}
% \vspace{-20pt}
\vspace{-10pt}
\noindent\rule{\dimexpr\columnwidth-2\fboxsep\relax}{0.8pt} % bottom rule
\end{algorithm}
 % bottom rule
% \vspace{-5pt}
}
